A Learning-based Quadcopter Controller with Extreme Adaptation

This paper introduces a learning-based low-level controller for quadcopters, which adaptively controls quadcopters with significant variations in mass, size, and actuator capabilities. Our approach leverages a combination of imitation learning and reinforcement learning, creating a fast-adapting and general control framework for quadcopters that eliminates the need for precise model estimation or manual tuning. The controller estimates a latent representation of the vehicle's system parameters from sensor-action history, enabling it to adapt swiftly to diverse dynamics. Extensive evaluations in simulation demonstrate the controller's ability to generalize to unseen quadcopter parameters, with an adaptation range up to 16 times broader than the training set. In real-world tests, the controller is successfully deployed on quadcopters with mass differences of 3.7 times and propeller constants varying by more than 100 times, while also showing rapid adaptation to disturbances such as off-center payloads and motor failures. These results highlight the potential of our controller in extreme adaptation to simplify the design process and enhance the reliability of autonomous drone operations in unpredictable environments. The video and code are at: https://github.com/muellerlab/xadapt_ctrl

==> sections/outline.tex <==
\section{Introduction}
\begin{itemize}
    \item cascade control takes a complex system and approximate it as a cascade of simpler nested systems.
    \item cascade control strategy has been widely used in quadcopters [cite] to decompose this system into nested subsystems which are easy to control.
    \item the cascade controller is constructed as follows (Fig1.A):
    \item the highest level control will control the vehicle's position and velocity with total thrust and attitude as inputs; the next level down is to control the attitude with angular velocities. The lowest level will control the angular velocities and total thrust with torques as inputs. The torques and total thrust could be linearly mapped to individual motor forces with the mixer matrix. 
    \item The controllers controlling position/ velocity/ attitude are referred as the high-level control which is general and invariant regarding quadcopter constants. 
    \item However, the low-level control which controls the angular velocity and maps torques to individual motor command requires explicit estimates of the vehicle's model, including inertia properties (mass and mass moment of inertia), motor constants, and other parameters.
    \item Errors in estimating such parameters directly translate to errors in the execution of the controller commands.
    \item In addition, once the parameters are estimated, the controller typically requires specific tuning in-flight to achieve the desired behaviour.
    \item A modification to the vehicle, e.g., replacing the motors with ones that have different properties, would require repeating the above steps in estimation and tuning.
    \item Such significant engineering efforts could be eased with a single controller without specialized tuning. 
    \item In our previous work, we show a single near-hover controller aiming to control a variety of quadcopters while able to rapidly adapt to unknown in-flight disturbances in the mass and inertia changes of the quadcopters.
    \item This controller is an end-to-end controller which controls the vehicle's position with individual motor speed as inputs. 
    \item We utilize the previous work and propose a pure low-level controller adaptive to vastly different quadcopters and to disturbances. This controller could augment with any high-level controller to control a variety of quadcopters without pre-tuning. (Fig1.B)
    \item More contribution: experience on learning a low-level high-frequency quadcopter control... 

    \item Fig1.A: traditional quadcopter cascade control diagram. Fig1. B: the control diagram for our controller use scenario 
\end{itemize}


\begin{itemize}
    \item Chronological literature review on adaptive control
\end{itemize}

\input{sections/related_work}

\section{Method}
\begin{itemize}
    \item We learn a single low-level controller to fly quadcopters
to track arbitrary trajectories. This controller takes historical data from
the onboard Inertial Measurement Unit (IMU) and commands
from a platform-independent, high level controller in the
cascade system as inputs and outputs individual motor speed.
    \item We extend the method RMA used in our previous work. 
\end{itemize}
\subsection{Base Policy}
\begin{itemize}
    \item We learn the base policy π in simulation using a mix of model-free
Reinforcement Learning (RL) and Behavior Cloning (BC). Inputs and outputs. 
    \item Base policy's network structure: MLP
    \item (a)Training quadcopter parameters range table 
    \item (b) Trajectory generation method: Mark's motion primitive paper
    \item \textbf{Excitation for online parameter estimation}
    \item (c) training details training procedure: at the beginning of training, use BC to clone a traditional PID controller for fast learning. gradually, the weight of the BC loss decrease and the weight of RL loss increase, so the training towards RL. 
    \item (d) RL Reward 
    \item \textbf{[practical tip:}. 
    \item (a)  Torque tracking: Show ablation studies of reward plot of torque tracking, and angular velocity tracking as one of reward metrics 
    \item (b) Training Episod Termination critiria: for example, angular velocity limit; the height of the drone in training 
\end{itemize}

\subsection{Adaptation Module}

\subsection{Deployment}
\begin{itemize}
    \item We directly deploy the base policy π which uses the current
state xt and the intrinsics vector ˆzt predicted by the adaptation
module φ. We do not calibrate or finetune our policy, and use
the same policy without any modifications on the different
drones under different payload and conditions.
    \item We convert pytorch model to MNN (cite) for running the low-level controller with quadcopter onboard computing unit. 
    \item the inference time is 0.1 ms. 
\end{itemize}


\input{sections/experiments}

\section{Conclusion}
